Synthesizing invariants by solving solvable loops

When proving invariance properties of a program, we face two problems. The first problem is related to the necessity of proving tautologies of considered assertion language, whereas the second manifests in the need of finding sufficiently strong invariants. This paper focuses on the second problem and describes a new method for the automatic generation of loop invariants that handles polynomial and non deterministic assignments. This technique is based on the eigenvector generation for a given linear transformation and on the polynomial optimization problem, which we implemented in the open-source tool Pilat.

==> codomain.tex <==
 \begin{Prop}

  
  $\exists \lambda, |\lambda| \geqslant 1, f^*(\varphi) = \lambda.\varphi \Rightarrow \varphi$ is a divergent semi-invariant 
\end{Prop}
 


==> codomain_proof.tex <==
\begin{proof}
If there exists $\lambda$ such that $f^*(\varphi) = \lambda.\varphi$, then we have that

\begin{equation*}
 |<\varphi,X>|~\geqslant~k \Rightarrow |<\varphi,f(X)>|~\geqslant~k
\end{equation*}

is equivalent to 

\begin{equation*}
 |<\varphi,X>|~\geqslant~k \Rightarrow |\lambda|.|<\varphi,X>|~\geqslant~k
\end{equation*}

If we also have that $|\lambda| > 1$, then the previous equation is true.
$\square$
\end{proof}


==> convergence.tex <==
 
\begin{Prop}\labelprop{convergence}
  Let $P$ and $Q$ two polynomials and $M>0 \in \mathbb{R}$. 
  
  If $\lim\limits_{\lVert X\rVert\rightarrow+\infty} |\frac{Q(X)}{P(X)}| < M$, then
  there exists $k \in \mathbb{R}$ such that for all $k' \geqslant k$
  
  \begin{equation*}
   |P(X)| \leqslant k' \Rightarrow |Q(X)|\leqslant M.k'
  \end{equation*}

\end{Prop}



==> convergence_proof.tex <==
\begin{proof}

  If $\lim\limits_{\lVert X\rVert\rightarrow+\infty} |\frac{Q(X)}{P(X)}| < N$, then
  there exists $X$ such that for all $X'$ with $\lVert X \rVert \leqslant \lVert X' \rVert$
  $ -N \leqslant \frac{Q(X)}{P(X)}\leqslant N$
   
  Let's now add the hypothesis $|P(X)| \leqslant k$.\\
  
  $-N  \leqslant\frac{Q(X)}{P(X)} \leqslant N  \Rightarrow  -N  \leqslant\frac{Q(X)}{k} \leqslant N$

  $\square$
\end{proof}
 


==> domain.tex <==
\begin{Prop}

 $\varphi$ is a convergent semi-invariant 
  $\Leftrightarrow
  \exists \lambda, |\lambda| \leqslant 1, f^*(\varphi) = \lambda.\varphi$
 
\end{Prop}


==> non_det_induction_equiv.tex <==
\begin{Prop}\labelprop{prop:nd_equiv_prop}
 
 $\forall X, |\scalprod{e_0}{X}| \leqslant k \Rightarrow |\lambda_0\scalprod{e_0}{X} + \scalprod{\delta_0^N}{X}| \leqslant k$~(\ref{eq:non_det})
 $\Leftrightarrow$ 
 
 \begin{equation}\label{eq:non_det_equiv}
\forall X, |\scalprod{e_0}{X}| \leqslant k \Rightarrow |\scalprod{\delta_0^N}{X}| \leqslant (1-|\lambda_0|).k
\end{equation}
\end{Prop}
 


==> non_det_induction_equiv_proof.tex <==
\begin{proof}
Let's focus on the right part of the implication (\ref{eq:non_det}) : 

\begin{eqnarray*}
&|\lambda_0\scalprod{e_0}{X} + \scalprod{\delta_0^N}{X}| &\leqslant k\\
-k \leqslant & \lambda_0\scalprod{e_0}{X} + \scalprod{\delta_0^N}{X} &\leqslant k\\
% - \lambda_0_0\scalprod{e_0}{X} - k \leqslant &\scalprod{\delta_0^N}{X} &\leqslant k - \lambda_0_0\scalprod{e_0}{X} \\
\end{eqnarray*}

Our hypothesis is $|\scalprod{e_0}{X}| \leqslant k$, which is equivalent to 
$-k \leqslant \scalprod{e_0}{X} \leqslant k$. 
% 

\begin{itemize}
 \item [$\bullet$] $\Leftarrow$
 
  If $\scalprod{\delta_0^N}{X} \leqslant (1-\lambda_0).k$, then  $\scalprod{\delta_0^N}{X} +\lambda_0.k \leqslant k$.
%   
  As $\lambda_0.\scalprod{e_0}{X} \leqslant \lambda_0.k$, we have $\lambda_0.\scalprod{e_0}{X} + \scalprod{\delta_0^N}{X} \leqslant \lambda_0 k + \scalprod{\delta_0^N}{X} \leqslant k$.

  ~
  
  Dually if $\scalprod{\delta_0^N}{X} \geqslant (\lambda_0-1).k$, then $\scalprod{\delta_0^N}{X} -\lambda_0.k \geqslant -k$.
%   
    As $\lambda_0.\scalprod{e_0}{X} \geqslant -\lambda_0.k$, we have $\lambda_0.\scalprod{e_0}{X} + \scalprod{\delta_0^N}{X} \geqslant \scalprod{\delta_0^N}{X} -\lambda_0.k \geqslant -k$.

 \item [$\bullet$] $\Rightarrow$
 
 We will perform a reasoning by the absurd. 
%  
 If there exist a $X$ such that 
 $\scalprod{\delta_0^N}{X} = (1-\lambda_0).k + \varepsilon$ with 
 $\varepsilon > 0$, then 
 $\lambda_0.\scalprod{e_0}{X} + \scalprod{\delta_0^N}{X} = \lambda_0.\scalprod{e_0}{X} + k - \lambda_0.k + \varepsilon$.
%  
 In the case where $\scalprod{e_0}{X} = k$ (which fits our hypotheses), $\lambda_0.\scalprod{e_0}{X} + \scalprod{\delta_0^N}{X} = k + \varepsilon > k$.
 
 Dually, if there exist a $X$ such that 
 $\scalprod{\delta_0^N}{X} = (\lambda_0-1).k - \varepsilon$ with 
 $\varepsilon > 0$, then 
 $\lambda_0.\scalprod{e_0}{X} + \scalprod{\delta_0^N}{X} = \lambda_0.\scalprod{e_0}{X} - k + \lambda_0.k - \varepsilon$.
%  
  
 In the case where $\scalprod{e_0}{X} = -k$ (which also fits our hypotheses), $\lambda_0.\scalprod{e_0}{X} + \scalprod{\delta_0^N}{X} = -k - \varepsilon < -k$.
\end{itemize}





 $\square$
 
\end{proof}
